Generalization Guarantees for Neural Architecture Search with Train-Validation Split

Neural Architecture Search (NAS) is a popular method for automatically designing optimized architectures for high-performance deep learning. In this approach, it is common to use bilevel optimization where one optimizes the model weights over the training data (inner problem) and various hyperparameters such as the configuration of the architecture over the validation data (outer problem). This paper explores the statistical aspects of such problems with train-validation splits. In practice, the inner problem is often overparameterized and can easily achieve zero loss. Thus, a-priori it seems impossible to distinguish the right hyperparameters based on training loss alone which motivates a better understanding of the role of train-validation split. To this aim this work establishes the following results. (1) We show that refined properties of the validation loss such as risk and hyper-gradients are indicative of those of the true test loss. This reveals that the outer problem helps select the most generalizable model and prevent overfitting with a near-minimal validation sample size. This is established for continuous search spaces which are relevant for differentiable schemes. Extensions to transfer learning are developed in terms of the mismatch between training & validation distributions. (2) We establish generalization bounds for NAS problems with an emphasis on an activation search problem. When optimized with gradient-descent, we show that the train-validation procedure returns the best (model, architecture) pair even if all architectures can perfectly fit the training data to achieve zero error. (3) Finally, we highlight connections between NAS, multiple kernel learning, and low-rank matrix learning. The latter leads to novel insights where the solution of the outer problem can be accurately learned via efficient spectral methods to achieve near-minimal risk.

==> app/fmap_proof.tex <==
\section{Proof of NTK-based NAS results}

==> app/nn_proof.tex <==
\section{Proof of Theorem \ref{one layer nas}}



==> app/proofs.tex <==
\section{Proofs of the Main Results}\label{sec:proof}

==> sec/main.tex <==
\section{Main Results}\label{sec:main}

==> sec/sec_local_gen.tex <==
\vs\vs
\section{Generalization with train-validation splits}\label{sec val gen}%Warm Up
In this section we state our generic generalization bounds for bilevel optimization problems with train-validation splits. Next, in Section \ref{sec:FMAP} we specialize these generic bounds to a feature map learning problem and a neural activation search problem. We begin by introducing the problem setting in Section \ref{probset}. We then introduce our first result in Section \ref{lowvalgen} which bounds the difference between the generalization and validation errors. Then in Section \ref{end2end} we relate train and validation errors which when combined with our first result yields an end-to-end generalization bound. 
%$ and the validation%\noindent\textbf{Notation:} 
\vs\vs
\subsection{Preliminaries and problem formulation}\label{probset}
We begin by introducing some notation used throughout the paper. We use $\X^\dagger$ to denote the Moore–Penrose inverse of a matrix $X$. $\gtrsim,\lesssim$ denote inequalities that hold up to an absolute constant. We define the norm $\lix{\cdot}$  over an input space $\Xc$ as $\lix{f}:=\sup_{\x\in\Xc} |f(\x)|$. $\ordet{\cdot}$ implies equality up to constant/logarithmic factors. $c,C>0$ are used to denote absolute constants. Finally, we use $\Ncov$ to denote an $\eps$-Euclidean ball cover of a set $\Bal$.
%$\te{\cdot}$ returns the sub-exponential norm of a random variable (cf.~Def.~5.13 of \cite{VERS}). 

% taking values over $\Xc\times \Yc$
Throughout, we use $(\x,y)\sim \Dc$ with $\x\in \Xc$ and $y\in\Yc$, to denote the data distribution of the feature/label pair. We also use $\Tc=\{(\x_i,y_i)\}_{i=1}^{\nt}$ to denote the training dataset and $\Vc=\{(\xt_i,\yt_i)\}_{i=1}^{\nv}$ the validation dataset and assume $\Tc$ and $\Vc$ are drawn i.i.d.~from $\Dc$. Given a loss function $\ell$ and a hypothesis $f:\Xc\rightarrow\Yc$, we define the population risk as $\Lc(f)=\E_{\Dc}[\ell(y,f(\x))]$ and the empirical training and validation risks as follows\vs
\[
\Lch_\Tc(f)=\frac{1}{\nt}\sum_{i=1}^{\nt} \ell(y_i,f(\x_i)),\text{ }\Lch_\Vc(f)=\frac{1}{\nv}\sum_{i=1}^{\nv} \ell(\yt_i,f(\xt_i)).
\]
For binary classification with $y\in\{-1,1\}$ also define the test classification error as $\Lcz(f)=\Pro(yf(\x)\leq 0)$. We focus on a \emph{bilevel empirical risk minimization} (ERM) problem over train/validation datasets involving a hyperparameter $\bal\in\R^\h$ and a hypothesis $f$. Here, the model $f$ (which depends on the hyperparameter $\bal$) is typically trained over the training data $\Tc$ with the hyperparameters fixed (inner problem). Then, the best hyperparameter is selected based on the validation data (outer problem). 

While the training of the inner problem is typically via optimizing an (possibly regularized) empirical loss of the form $\Lch_\Tc$, we do not explicitly require a global optima of this empirical loss and assume that we have access to an algorithm $\Ac$ that returns a model based on the training data $\Tc$ with hyperparameters fixed at $\bal$ %$\Lch_\Tc$. $\Ac(\cdot,\cdot)$. $\Ac$ admits $\bal$ and training data $\Tc$ as input and outputs a unique hypothesis $\ft_\bal$ as follows\
\[\vs
\ft_\bal=\Ac(\bal,\Tc).\vs
\]
We provide some example scenarios with the corresponding algorithm below.

\noindent\emph{Scenario 1: Strongly Convex Problems.} The Inner problem ERM is strongly convex with respect to the parameters of the model and $\Ac$ returns its unique solution. A specific example is learning the optimal kernel given a predefined set of kernels per \S\ref{sec:FMAPsec}. 
%This is the topic of Section \ref{sec:FMAP}.
%Examples include ridge regression or min-norm interpolation.

\noindent\emph{Scenario 2: Gradient Descent \& NAS.} In NAS, $f$ is typically a neural network and $\bal$ encodes the network architecture. Given this architecture, starting from randomly initialized weights, $\Ac$ trains the weights of $f$ on dataset $\Tc$ by running fixed number of gradient descent iterations. See \S\ref{sec:NAS} and \S\ref{sec deep} for more details. 

As mentioned earlier, modern NAS problems typically obey \eqref{roi eq} where the inner problem involves fitting an overparameterized network with many parameters whereas the number of architectural parameters $\h$ is typically less than 1000 and obeys $\h=\text{dim}(\bal)\leq \nv$. Intuitively, this is the regime in which any inner problem can perfectly fit the data. However, the under-parameterized outer problem can potentially guide the algorithm towards the right model. Our goal is to provide theoretical insights for this regime. To select the optimal model, given hyperparameter space $\Bal$ and tolerance $\del>0$, we consider a $\del$-approximate solution to the empirical risk over the validation data $\Lch_\Vc$ (outer problem)\vs
\begin{align}%\tag{BL-ERM} % Consider adding a $\text{comp}(\bal)$ penalty...
&\bah\in \{\bal\in\Bal\bgl \Lch_\Vc(\ft_\bal)\leq \min_{\bal\in\Bal}\Lch_{\Vc}(\ft_\bal)+\del\} \label{opt alpha}.
%\\&\clr{\bah\in \{\bal\in\Bal\bgl \Lch_\Vc(\ft_\bal)+\text{Comp}(\bal)\leq \min_{\bal\in\Bal}\Lch_{\Vc}(\ft_\bal)+\text{Comp}(\bal)+\del\}}\nn
\end{align}\vs\vs\vs\vs
\vs\vs
\subsection{Low validation risk implies good generalization}\label{lowvalgen}
Our first result connects the test (generalization) error to that of the validation error. A key aspect of our result is that we establish uniform convergence guarantees that hold over continuous hyperparameter spaces which is insightful for differentiable HPO/NAS algorithms such as DARTS \cite{liu2018darts}. Our results rely on the following definition and assumptions. 
\vs
\begin{definition} [Effective dimension] \label{cover assump} For a set $\Bal\in\R^\h$ of hyperparameters we define its effective dimension $\deff$ as the smallest value of $\deff>0$ such that $\abs{\Ncov}\le ({\bC}/{\eps})^{\deff}$ for all $\eps>0$ and a constant $\bC>0$.
%and $\bC>0$ such that $\eps$-Euclidian norm covering number of $\Bal$ is upper bounded by $({\bC}/{\eps})^{\deff}$. $\Ncov$
\end{definition}\vs\vs
The effective dimension captures the degrees of freedom of a set $\Bal$. In particular, if $\Bal\in\R^\h$ has Euclidian radius $R$, then $\deff=\h$ with $\bC=3R$ so that it reduces to the number of hyperparameters. However, $\deff$ is more nuanced and can also help incorporate problem structure/prior knowledge (e.g.~sparse neural architectures have less degrees of freedom). \vs
\begin{assumption} \label{algo lip} $\Ac(\cdot)$ is an $L$-Lipschitz function of $\bal$ in $\lix{\cdot}$ norm, that is, for all pairs $\bal,\bal'\in \Bal$ with $\tn{\bal-\bal'}\leq \eps$, we have $\lix{\ft_\bal-\ft_{\bal'}}\leq L\eps$.
\end{assumption}\vs\vs

\begin{assumption}\label{loss assump}For all hypotheses $\ft_\bal$, the loss $\ell(y,\cdot)$ is $\Gamma$-Lipschitz over the feasible set $\{\ft_\bal(\x)\bgl \x\in\Xc\}$.
\end{assumption}\vs
\begin{definition}[Risk growth function] On a point $\bal\in\Ac$, let $S_\bal$ be the $\ell(y,\ft_\bal(\x))-\E[\ell(y,\ft_\bal(\x))]$ subexponential ($\|\cdot\|_{\psi_1}$) norm with respect to the randomness in $(\x,y)\sim\Dc$. The error growth function is defined as
\[
\Gc(\bal)=\left(\Lc(\ft_{\bal})-\min_{\bal\in\Bal}\Lc(\ft_{\bal})\right)-C\sqrt{\frac{S_\bal(\defz+\tau)}{\nv}}
\]
\end{definition}\vs
Assumption \ref{algo lip} is key to our NAS generalization analysis and we show it holds in a variety of scenarios. Assumption \ref{loss assump} requires the loss $\ell$ to have a sub-exponential tail. Our first result establishes a generalization guarantee for \eqref{opt alpha} under these assumptions.% which applies to % sholds for bounded losses but can also be applied to unbounded ones.
%\cln{The lemma below provides a simple condition for which this assumption holds.
%\begin{lemma} Let $\bt\in\R^p$ be the parameterization of the hypothesis $f$ i.e.~$f(\x)=f(\x,\bt)$. Suppose inner problem is $\mu$-strongly convex over $\bt$ and $\Ac$ returns its unique solution. Suppose outer problem is $L$-smooth. Then $\tn{\bt_\bal-\bt_{\bal'}}\leq \sqrt{L/\mu}\tn{\bal-\bal'}$.
%\end{lemma}
%This lemma implies the Lispchitzness of the model weights in terms of hyperparameters.}
%uniform convergence analysis and can be verified for % \cite{VERS}.
%assume that the set $\Bal$ has a favorable covering number, $\Ac$ is Lipschitz, and $\ell$ behaves nicely.
%Let $\Gamma>0$ be an upper bound on the Lipschitz constant of $\ell(y,\cdot)$ over the set of all feasible predictions $\hat{y}=\ft_\bal(\x)$. Additionally, suppose $(\x,y)\sim\Dc$ induce a $\Gamma$-subexponential loss i.e.~for any fixed $f$ (induced by some $\bal\in\Bal$), $\te{\ell(y,f(\x))-\E[\ell(y,f(\x))]}\leq \Gamma$.
%Suppose the elements of $\Xc,\Yc$ have $\ell_2$ norms bounded by $B_x,B_y$. 
%Let $\Dc$ be the data distribution taking values over $\Xc\times \Yc$. 
%[Uniform Convergence over Validation] 
\vs
\begin{theorem}\label{thm val} Suppose Assumptions \ref{algo lip}-\ref{loss assump} hold.  Let $\bah$ be an approximate minimizer of the empirical validation risk per \eqref{opt alpha} and set $\defz:=\deff\log(2\bC L\Gamma \nv/\deff)$. Also assume $\nv\geq C(\defz+\tau)$ for a constant $C>0$ and some $\tau> 0$. Then,
%\begin{align}
%&\Lc(f_{\bah})\leq \inf_{\bal\in \Bal}\Lc(f_\bal)+ 2\sqrt{C}\frac{\sqrt{\defz+\tau}}{\sqrt{\nv}}+\del\quad\text{and}\quad\Lc(f_{\bah})\leq \min_{\bal}\Lch_{\Vc}(f_\bal)+\sqrt{C}\frac{\sqrt{\defz+\tau}}{\sqrt{\nv}}+\del.\label{stronger eq}
%\end{align}
\vs\vs\begin{align}
%&\Lc(\ft_{\bah})\leq \min_{\bal}\Lch_{\Vc}(\ft_\bal)+\sqrt{C(\defz+\tau)/\nv}+\del\label{eval1}\\
\sup_{\bal\in\Bal}|\Lc(\ft_{\bal})- \Lch_{\Vc}(\ft_\bal)|\leq&\sqrt{\frac{C(\defz+\tau)}{\nv}}+\del\label{eval1},\\
\Lc(\ft_\bah)\leq \min_{\bal\in \Bal}\Lc(\ft_\bal)+2&\sqrt{\frac{C(\defz+\tau)}{\nv}}+\delta.\label{excess risk val}
\end{align}\vs
hold with probability at least $1-2e^{-\tau}$ .
\end{theorem}\vs\vs
%\noindent\textbf{Interpretation:} 
This result shows that as soon as the size of the validation data exceeds the effective number of hyperparameters $\nv\gtrsim \h$ (up to log factors) then (1) as evident per \eqref{eval1} the test error is close to the validation error (i.e.~validation error is indicative of the test error) and (2) per \eqref{excess risk val} the optimization over validation is guaranteed to return a hypothesis on par with the best choice of hyperparameters in $\Bal$. We note that \eqref{excess risk val} follows from \eqref{eval1} via a uniform convergence argument. We also note that when $\Bal$ is a discrete set, a standard union bound would require $\nv\propto\log|\Bal|$ samples. Thus the key contribution of this result is that it applies to continuous hyperparameters and bounds the size of $\Bal$ via the more refined notion of effective dimension, establishing a logarithmic dependence on problem parameters. This is particularly important in the case of $L$ which can be rather large in practice. %This result shows that as long as $L,\Gamma$ are not exponentially large, we establish uniform convergence over continuous hyperparameters with few samples. 
%\clr{We note that there is additional logarithmic dependency $\nv/\deff$. Fortunately, this dependency becomes negligible in the small data regime where $\nt\propto \h$.}
%\noindent\textbf{Remark:} 
Finally, we note that Assumption \ref{algo lip} can be replaced with a weaker Lipschitz approximation condition where $\ft_\bal$ itself is not $L$-Lipschitz but is approximately close to an $L$-Lipschitz function (cf.~Theorem \ref{thm val2} in the supplementary). 

%s $g_\bal$ such that $\lix{g_\bal-\ft_\bal}\leq\eps$ for all $\bal\in\Bal$. Then, statement of Theorem \ref{thm val} remains same after increasing the risk bounds by $8\eps\Gamma$ (see SM). This observation is in fact helpful later on for our NAS guarantees.% is in fact how we address neural nets later on.

Finally, we note that the results above do not directly imply good generalization as they do not guarantee that the validation error ($\min_{\bal}\Lch_{\Vc}(\ft_\bal)$) or the generalization error ($\min_{\bal\in \Bal}\Lc(\ft_\bal)$) of the model trained with the best hyperparameters is small. This is to be expected as when there are very few training data one can not hope for the model $\ft_\bal$ to have good generalization even with optimal hyperparameters. However, whether the training phase is successful or not, the validation phase returns approximately the best hyperparameters even with a bad model! In the next section we do in fact show that with enough training data the validation/generalization of the model trained with the best hyperparameter is indeed small allowing us to establish an end-to-end generalization bound.

\subsection{\small{End-to-end generalization with Train-Validation Splits}}\label{end2end}% Given distribution $\Dc$ as its input, suppose $\Ac$ returns the population hypothesis $\fs$
We begin by briefly discussing the role of the training data which is necessary for establishing an end-to-end bound. To this aim, we need to characterize how the population loss of the algorithm $\Ac$ scales with the training data $\nt$. To this aim, let us consider the limiting case $\nt\rightarrow +\infty$ and define the corresponding model for a given set of hyperparameters $\bal$ as
\[
\fs_\bal:=\Ac(\bal,\Dc):=\lim_{\nt\rightarrow\infty} \Ac(\bal,\Tc).
\]
Classical learning theory results typically bound the difference between the population loss/risk of a model that is trained with finite training data ($\Lc(\ft_\bal)$) and the loss achieved by the idealized infinite data model ($\Lc(\fs_\bal)$) in terms of an appropriate complexity measure of the class and the size of the training data.
%Also define the generalization gap $\exc{\Tc}:=\inf_{\bal\in \Bal}\Lc(\ft_\bal)-\inf_{\bal\in \Bal}\Lc(\fs_\bal)$. Plugging this in \eqref{excess risk val} gives
%\[
%\Lc(\ft_\bah)\leq \inf_{\bal\in \Bal}\Lc(\fs_\bal)+\exc{\Tc}+2\sqrt{C(\defz+\tau)/\nv}+\delta.
%\]%is that, 
%To proceed, let us bound the $\exc{\Tc}$ in terms of the sample size $\nt$. 
In particular, for a specific choice of the hyperparameter $\bal$, based on classical learning theory \cite{bartlett2002rademacher}) a typical behavior is to have
\vs\begin{align}
\Lc(\ft_\bal)\leq \Lc(\fs_\bal)+\frac{\Cc_\bal^\Tc+C_0\sqrt{t}}{\sqrt{\nt}}.\label{unif alll}
%\Lc(\ft_\bal)\leq \Lc(\fs_\bal)+\frac{\Cc_\bal}{\sqrt{\nt}},
\vs\end{align}
with probability at least $1-\e^{-t}$. Here, $\Cc_\bal^\Tc$ is a data dependent complexity measure for the hypothesis set of the inner problem and $C_0>0$ is a scalar. We are now ready to state our end-to-end bound which ensures a bound of the form \eqref{unif alll} holds simultaneously for all choices of the hyperparameter $\bal\in\Bal$. %Consider stating for $\Bas$.
%One can upper bound the right hand side uniformly over all $\bal$ inner training risk uniformly over all $\bal$ under mild conditions.
%\clr{Note that, standard bounds hold only for a particular choice of $\bal$. In our approach --discussed subsequently-- we also upper bound this inner training risk uniformly over all $\bal$ under mild conditions.}
%\begin{assumption} \label{assump star}Assume $\fs_\bal$ (in $\|\cdot\|_{\Xc}$ norm) and $\Cc_\bal$ have bounded Lipschitz constants with respect to $\bal$ over $\Bal$. 
%There exists a domain $\Bal_\st\subset \Bal$ and some $\bL>0$ such that $\fs_\bal$ (in $\|\cdot\|_{\Xc}$ norm) and the excess risk term $\Cc_\bal$ are $\bL$-Lipschitz function of $\bal$. 
%\end{assumption}
\vs
\begin{proposition} [Train-validation bound] \label{unif excess lem} Consider the setting of Theorem \ref{thm val} and for any fixed $\bal\in\Bal$ assume \eqref{unif alll} holds. Also assume $\fs_\bal$ (in $\|\cdot\|_{\Xc}$ norm) and $\Cc_\bal^\Tc$ have bounded Lipschitz constants with respect to $\bal$ over $\Bal$. Then with probability at least $1-4\e^{-t}$ over $\Tc$~and~$\Vc$ datasets
\vs\begin{align}
\Lc(\ft_\bah)\leq \min_{\bal\in\Bal}\left(\Lc(\fs_\bal)+\frac{\Cc_\bal^\Tc}{\sqrt{\nt}}\right)+\sqrt{\frac{\ordet{\deff+t}}{\nv}}+\delta.\nn%\label{abcdef}
\end{align}\vs%\log(L+\bL)
\end{proposition}\vs
%With this, we end up with a bound over $\Tc$ and $\Vc$ by upper bounding $\exc{\Tc}$ via $\inf_{\bal\in \Bal_\st}\Lc(\ft_\bal)-\inf_{\bal\in \Bal_\st}\Lc(\fs_\bal)$.

In a nutshell, the above bound shows that the generalization error of a model trained with train-validation splits is on par with the best train-only generalization achievable by picking the best hyperparameter $\bal\in\Bal$. The only loss incurred is an extra $\sqrt{\deff/\nv}$ term which is vanishingly small as soon as the validation data is sufficiently larger than the effective dimension of the hyperparameters. In the next section, we demonstrate how we can utilize this end-to-end guarantee in specific domains.%Assumption \ref{assump star} will be helpful in \S\ref{sec deep} where generalization bounds may apply only for a subset of deep nets.

%\cln{We will assume the generalization performance is captured by an excess risk function $\exc{\nt,t}$.% which admits an $(f,\bal)$ pair.
%\begin{assumption} \label{assump excess} There exists $\bal\in\Bal$ such that Algorithm $\Ac$ trained over $\Tc$ satisfies the generalization bound $\Lc(\ft_\bal)\leq \min_{\bal\in\Bal}\Lc(\fs_\bal)+\exc{\nt,t}$ with probability $1-\e^{-t}$.
%%\[\tsn{\ft_\bal,\bal}+\frac{g(\bal)t}{\sqrt{\nt}}.\]
%\end{assumption}
%When verifying this assumption in practice, an intuitive choice for $\bal$ is using the optimal population parameter $\bas=\arg\min_{\bal\in\Bal}\Lc(\fs_\bal)$. Secondly, note that $\exc{\nt,t}$ term is typically decreases as $1/\sqrt{\nt}$.
%\begin{corollary}[End-to-end learning bound] Suppose Assumptions \ref{cover assump}, \ref{algo lip}, \ref{loss assump}, \ref{assump excess} hold. With probability $1-2\e^{-t}$, we have that
%\[
%\Lc(f_{\bah})\leq \min_{\bal\in \Bal}\Lc(\fs_\bal)+\exc{\nt,t}+2\sqrt{C}\frac{\sqrt{\defz+t}}{\sqrt{\nv}}.\label{excess risk val}
%\]
%\end{corollary}
%For the proof, observe that Assumption 4 implies that $\min_{\bal\in \Bal}\Lc(\ft_\bal)\leq \min_{\bal\in \Bal}\Lc(\fs_\bal)+\exc{\nt,t}$ with probability $1-\e^{-t}$. }






==> sec/setup_NAS.tex <==
\section{Problem Setup}\label{sec:setup}

\noindent\textbf{Notation:} 

Let us start with providing necessary background on NAS and its connection to matrix factorization. Consider a feedforward DNN which can be represented as a directed acyclic graph. The nodes of this graph corresponds to the hidden feature representations of the input and the edges in between corresponds to the functions connecting them. Mathematically, the $j$th hidden features $\x^{(j)}$ are obtained using previous features via $\x^{(j)}=\sum_{i<j}f^{(i,j)}(\x^{(i)})$ where $f^{(i,j)}$ is the function connecting the nodes. In NAS, $f^{(i,j)}$ encodes the weight matrix $\bt^{(i,j)}$ and the high-level operation to use (e.g.~conv vs max-pool). In Differentiable NAS, each operation is in the span of a finite pre-defined set and we use its vector representation, say $\bal^{(i,j)}$, obtained via one-hot encoding. Collecting these vectors (for all $(i,j)$) in $(\bal,\bt)$ respectively, and denoting the prediction function by $\fab$ our goal is minimizing the risk $\E_{\Dc}[\ell(y,\fab(\x))]$ where $(\x,y)\sim\Dc$ is the data and $\ell$ is a loss function.

\noindent\textbf{Connection to kernels and matrix factorization:} Recent works prove deep connections between DNNs and kernels. The core idea is that sufficiently wide DNNs have approximately linear training dynamics, specifically, we have that% $\fab(\x)\approx \faz(\x)+\frac{\partial\faz(\x)}{\partial\bt} (\bt-\bt_0)$
\[
\fab(\x)\approx\li\phi_{\bal}(\x), \bt\ri,%\approx \li\phi_{\bal}(\x), \bt-\bt_0\ri
\]
where $\phi_\bal$ is the feature map induced by the linearized neural net (i.e.~neural tangent kernel). While this exposition is standard, the architecture is critical to our setup and it controls the quality of the kernel hence the eventual performance. For a DNN, $\phi_{\bal}$ is a nonlinear function of $\bal$ however, for a simple two-layer DNN, the dependency is linear. 

\textbf{Example: Activation search.} Denote input and output layer weights $\w\in\R^k,\W\in\R^{k\times d}$ respectively and set $\bt=[\w,\W]$. Also let $\Phi=(\rho_i)_{i=1}^q$ be set of activation functions. Consider a network $f^\bal_\bt(\x)=\w^T\rho_\bal(\W\x)$. Here activation function $\rho_\bal$ is given by the combination $\rho_\bal=\sum_{i=1}^q\bal_i\rho_i$. Linearization of the network induces the NTK kernel. This kernel is induced by the feature map calculated at the initialization $(\w_0,\W_0)$
\[
\phi_\bal(\x)=\begin{bmatrix}\rho_\bal(\W_0\x)\\\w_0\otimes \rho_\bal'(\W_0\x)\end{bmatrix}.
\]
This implies that for a one-hidden layer network, the feature maps are linear functions of $\bal$. Specifically, each feature map can be written as
\[
\phi_\bal(\x)=\Phi_{\x}^T\bal\quad\text{where}\quad \Phi_{\x}=\begin{bmatrix}\phi_1(\x)~\dots~\phi_q(\x)\end{bmatrix}^T\in\R^{q\times p}
\]
With this exposition, the output of the neural net takes the form 
\[
\fab(\x)\approx \bal^T\Phi_{\x}\bt.
\]
We wish to find the optimal $\bal,\bt$ pair minimizing the risk
\[
\Lc(\bal,\bt)=\min_{\bal,\bt} \sum_{i=1}^n \ell(y_i,\bal^T\X_i\bt).
\]
where we used the short hand notation $\X_i:=\Phi_{\x_i}$.

\textbf{Connection to Low-rank Regression.} This also reveals the connection to rank-1 matrix regression. Specifically, the problem above is equivalent to learning a rank-1 matrix $\M=\bal\bt^T\in\R^{q\times p}$ such that $y_i\approx \li\M,\X_i\ri$.

\textbf{Overparameterization.} The traditional literature on low-rank regression, Burer-Monteiro factorization and phase-retrieval assumes that sample size is larger than the degrees of freedom of the problem, that is $n\gtrsim p+q$. In contrast, neural nets operate in the opposite regime where the model tends to be overparameterized i.e.~$p>n$. Unfortunately, this regime makes learning very difficult for standard empirical risk minimization. The reason is simple: For any arbitrary choice of $\bal$, as long as the $\bal$-induced feature matrix $\X_\bal=[\phi_\bal(\x_1)~\dots~\phi_\bal(\x_n)]^T$ is full rank - which holds under very mild assumptions, $\bt$ will perfectly interpolate and ERM will achieve zero risk. This means that simply minimizing ERM have no business learning $\bal$!
 
%\textbf{TODO:} Introduce matrix-factor, activation search, justify p>n>c

% is used to map a discrete set of operations to vectors  $\bal^{(i,j)}$ is a vector encoding the actual operation.
\newpage

A feedforward DNN can be represented as a directed acyclic graph. The nodes of this graph corresponds to the hidden feature representations of the input and the edges in between corresponds to the functions connecting them. Mathematically, the $j$th hidden features $\x^{(j)}$ are obtained using previous features via $\x^{(j)}=\sum_{i<j}o^{(i,j)}(\x^{(i)})$ where $o^{(i,j)}$ is the function connecting the nodes. Here, $o^{(i,j)}$ encodes the weight matrix and the high-level operation to use (e.g.~convolution vs max-pooling) \cite{pham2018efficient,li2019random}. This operation is chosen from a pre-defined $\Phi=\{\phi_k\}_{k=1}^{|\Phi|}$. As visualized in Fig.~\ref{fig:NASprune}, for a fully-connected network, an instructive problem is {\em{jointly optimizing the activation function and weights}} where we write $\x^{(j)}=\sum_{i<j}\phi^{(i,j)}(\W^{(i,j)}\x^{(i)})$ with $\phi^{(i,j)}$ being the activation function. For instance, $\Phi$ can be $\{\text{relu},\text{sigmoid},\text{identity},\text{zero}\}$ as in Fig.~\ref{fig_main}. The {\em{zero activation}} means $\W^{(i,j)}$ can be removed and promotes inference-time efficiency in synergy with Task 2. While the original problem is a discrete search, gradient-based techniques can be employed via continuous relaxation \cite{liu2018darts} by parameterizing the target activation via $\phi^{(i,j)}(x)=\sum_{i=1}^{|\Phi|} \alpha^{(i,j)}_k \phi_k(x)$ where $\alpha_k$ typically admits a simplex constrain $\alpha_k\geq 0,~\sum_{k=1}^{|\Phi|}\alpha_k=1$. With this parameterization, the architecture configuration in \eqref{bl eq} is given by $\bal=\{ \alpha^{(i,j)}_k\}$. In what follows, the validation dataset is denoted by $\Vc=(\x'_i,y'_i)_{i=1}^v$ and the configuration $\bal$ is $c$ dimensional.


This task will study the optimization dynamics and statistical performance of \ref{bl eq} with an emphasis on NAS. We will first establish a link between NAS and rank-1 matrices.

\noindent$\bullet$ {\textbf{Task 3a.1: Bilevel Matrix Factorization.}} Consider the linear approximation \eqref{tay eq} of a DNN with architecture configuration $\bal$ which induces a feature map $\psi_{\bal}$. Thus, we are searching for the optimal kernel (feature map) over a space $\Ac$ which connects NAS to the multiple kernel learning problem \cite{sonnenburg2006large,bach2004multiple}. While $\psi_{\bal}$ is a nonlinear function of $\bal$ for deep networks, when network has a single hidden-layer, it can be written as $\psi_{\bal}=\sum_{i=1}^K\alpha_i\psi_i$. In matrix notation, given an input $\x_i$, consider the feature matrix $\X_i=[\psi_1(\x_i)~\dots~\psi_K(\x_i)]$. The linearized model output can be written compactly via $f_{\bt,\bal}(\x)\approx\bt^T\X\bal$. Thus, the problem takes a neat form where our goal is finding the optimal rank-1 matrix $\M=\bt\bal^T$ to minimize \ref{bl eq} over the data $\Sc,\Vc$. What are the provable statistical and optimization benefits of this problem? A {\em{baseline approach}} to compare \ref{bl eq} is merging $\Sc$ and $\Vc$ and jointly optimizing $(\bal,\bt)$ by solving \ref{erm eq}. In Fig.~\ref{fig:bilevel} we compare these by solving both with alternating least-squares on an exact planted model $y_i=\bt_\st^T\X_i\bal_\st$ (with $\X_i$ i.i.d.~entries). When the problem is under-parameterized, both approaches work well however under growing $p$ and over-parameterization \ref{erm eq} fails whereas \ref{bl eq} is robust. 
